Geometry of Reachability sets of Vector Addition Systems

Vector Addition Systems (VAS), aka Petri nets, are a popular model of concurrency. The reachability set of a VAS is the set of configurations reachable from the initial configuration. Leroux has studied the geometric properties of VAS reachability sets, and used them to derive decision procedures for important analysis problems. In this paper we continue the geometric study of reachability sets. We show that every reachability set admits a finite decomposition into disjoint almost hybridlinear sets enjoying nice geometric properties. Further, we prove that the decomposition of the reachability set of a given VAS is effectively computable. As a corollary, we derive a simple algorithm for deciding semilinearity of VAS reachability sets, the first one since Hauschildt's 1990 algorithm. As a second corollary, we prove that the complement of a reachability set always contains an infinite linear set.

==> Full_Linear_sets.tex <==
% !TeX root = geometry_of_VAS.tex

We introduce full linear sets, which were indirectly used already in \cite{Leroux13} and \cite{Leroux11}. 

Previous Usage of full linear sets: [10] introduces an overapproximation Lin(P) of a periodic set P that is equivalent to our Fill(P).  (In [11] and [12], the same author used the same notation with a different meaning; to avoid confusion we write Fill(P) instead.) In particular, Proposition 4.6 of our paper corresponds to Lemma 5.1 of [10]. However, [10]-[12] do not give a name to the class of periodic sets that are equal to their overapproximations. So full sets were not directly introduced in [10]-[12], but they were used indirectly. 

%The main goal is better geometric intuition. As proof of concept, we show that the corresponding class of full semilinear sets actually coincides with the semilinear sets, i.e. if done correctly, we avoid loss of information.

A periodic set \(\vect{P}\) induces a cone \(\mathbb{Q}_{\geq 0}\vect{P}\) and a lattice \(\vect{P}-\vect{P}\). Intuitively, the cone gives information about the region of the space containing $\vect{P}$, and the lattice describes ``modulo data'', like ``only even valued points of the cone are in \(\vect{P}\)''. Ideally, one would like to have \(\vect{P}= (\vect{P}-\vect{P}) \cap \mathbb{Q}_{\geq 0}\vect{P}\), but this is not always the case even for finitely generated periodic sets. Intuitively, the reason is that $\vect{P}$ may contain ``holes''. For example, consider the set $\vect{P}$ in the middle of Figure \ref{Fig:ExampleFullLinearSet}. The points of the form \((x,1)\) are ``holes'' in $\vect{P}$.

\begin{definition}
\label{def:fill}
Let $\vect{P}$ be a periodic set. The \emph{fill} of $\vect{P}$ is the set \(\Fill(\vect{P}):=(\vect{P}-\vect{P}) \cap \overline{\mathbb{Q}_{\geq 0}\vect{P}}\).  A periodic set $\vect{P}$ or linear set $\vect{b}+\vect{P}$ is \emph{full} if \(\overline{\Q_{\geq 0}\vect{P}}\) is finitely generated and \(\vect{P}=\Fill(\vect{P})\). 
\end{definition}

The reason for using the closure of $\mathbb{Q}_{\geq 0}\vect{P}$ instead of the cone $\mathbb{Q}_{\geq 0}\vect{P}$ itself is Lemma \ref{LemmaCharactizeFinitelyGeneratedPeriodicSets}: If the cone is not closed, then the periodic set, in our case \(\Fill(\vect{P})\), is not finitely generated. If \(\vect{P}\) was already finitely generated, the definitions coincide.

The following three lemmas collect some useful elementary properties of the fill, similar to properties from \cite{Leroux13} or very simple; proofs are in the appendix. Illustrations are in Figure \ref{Fig:ExampleFullLinearSet}.

\begin{restatable}{lemma}{FullAfterFill}
Let \(\vect{P}\) be a periodic set. Then \(\Fill(\Fill(\vect{P}))=\Fill(\vect{P})\). \label{LemmaFullAfterFill}
\end{restatable}

\begin{restatable}{lemma}{LemmaLatticeEqualsMonoid}
Let \(\vect{P}\) be a finitely generated periodic set. There exists \(\vect{x}\in \vect{P}\) such that \(\vect{x}+\Fill(\vect{P}) \subseteq \vect{P}\). \label{LemmaLatticeEqualsMonoid}
\end{restatable}

%It should be mentioned that this lemma is a generalization of a well-known result in dimension 1 to higher dimensions. In dimension 1, given any set \(F \subseteq \N\) with \(\gcd(F)=1\), there is some constant \(c\) such that every number \(m \geq c\) fulfills \(m\in F^{\ast}\). For example with packaging sizes \(3\) and \(5\), every number of objects greater than or equal to 8 can be packaged.

\begin{restatable}{lemma}{LemmaRemovingInnerConeReducesDimension}
Let \(\vect{P}\) be a finitely generated periodic set. For every \(\vect{x} \in \vect{P}\) the set \(\vect{S}:=\vect{P} \setminus (\vect{x} + \Fill(\vect{P}))\) is semilinear and satisfies \(\dim(\vect{S}) < \dim(\vect{P})\). \label{LemmaRemovingInnerConeReducesDimension}
\end{restatable}

%This lemma allows induction on dimension, and will be used frequently also in later sections. 

The lemmas lead to the main result of this section: Every semilinear set is a finite union of \emph{full} linear sets. In other words, the restriction to full sets does not decrease the ``expressive power'' of linear sets. 

\begin{proposition}
Let \(\vect{S}\) be a semilinear set. Then there exist full linear sets \(\vect{S}_i\) such that \(\vect{S}=\bigcup_{i=1}^r \vect{S}_i\). In addition, we can require \(\vect{S}_i \cap \vect{S}_j=\emptyset\) for all \(i\neq j\). \label{PropositionGoodSemilinearRepresentation}
\end{proposition}

\begin{proof}
Proof by induction on \(\dim(\vect{S})\). Write \(\vect{S}=\bigcup_{i=1}^r \vect{L}_i\) with linear sets \(\vect{L}_i\) such that \(\vect{L}_i \cap \vect{L}_j =\emptyset\) for all \(i,j\). The claim holds for \(\vect{S}\) if it holds for all \(\vect{L}_i\). Hence assume w.l.o.g. \(\vect{S}\) linear, i.e. \(\vect{S}=\vect{b}+\vect{P}\) for \(\vect{b}\in \N^n\) and \(\vect{P}\) finitely generated periodic set. By Lemma \ref{LemmaLatticeEqualsMonoid} we obtain a vector \(\vect{x} \in \vect{P}\) such that \(\vect{x} + \Fill(\vect{P}) \subseteq \vect{P}\). By Lemma \ref{LemmaRemovingInnerConeReducesDimension}, we obtain that \(\vect{S} \setminus (\vect{x}+\Fill(\vect{P}))\) is semilinear with a lower dimension, therefore by induction it can be written as a finite union as required. By simply adding \(\vect{x}+\Fill(\vect{P})\) to this representation, we obtain the required representation for \(\vect{S}\).
\end{proof}

However, this class is not only visually pleasing, it also has mathematical advantages. Lemma \ref{LemmaEquivalentDefinitionOfFull} provides an equivalent condition for membership in this class, and Lemma \ref{LemmaFullThenLessPeriods} proves a useful property which unintuitively is false even for finitely generated periodic sets.

\begin{restatable}{lemma}{LemmaEquivalentDefinitionOfFull}
Let \(\vect{C}\) be a finitely generated cone, \(\vect{L}\) a lattice. Then \(\vect{P}:=\vect{C}\cap \vect{L}\) is full. \label{LemmaEquivalentDefinitionOfFull}
\end{restatable}

\begin{restatable}{lemma}{LemmaFullThenLessPeriods}
Let \(\vect{P},\vect{Q}\) be periodic sets, \(\vect{P}\) full, and \(\vect{b},\vect{c} \in \Q^n\) points such that \(\vect{c}+\vect{Q} \subseteq \vect{b}+\vect{P}\). Then \(\vect{Q} \subseteq \vect{P}\). In particular, the representation \(\vect{b}+\vect{P}\) of a full linear set is unique. \label{LemmaFullThenLessPeriods}
\end{restatable}

Observe that if \(\vect{P}\) is the periodic set in the middle of Figure \ref{Fig:ExampleFullLinearSet}, then \((2,3)+\{(1,1)\}^{\ast} \subseteq \vect{P}\), and the property is violated, since \((1,1) \not \in \vect{P}\).
